VRDSynth: Synthesizing Programs for Multilingual Visually Rich Document Information Extraction

Businesses need to query visually rich documents (VRDs) like receipts, medical records, and insurance forms to make decisions. Existing techniques for extracting entities from VRDs struggle with new layouts or require extensive pre-training data. We introduce VRDSynth, a program synthesis method to automatically extract entity relations from multilingual VRDs without pre-training data. To capture the complexity of VRD domain, we design a domain-specific language (DSL) to capture spatial and textual relations to describe the synthesized programs. Along with this, we also derive a new synthesis algorithm utilizing frequent spatial relations, search space pruning, and a combination of positive, negative, and exclusive programs to improve coverage. We evaluate VRDSynth on the FUNSD and XFUND benchmarks for semantic entity linking, consisting of 1,592 forms in 8 languages. VRDSynth outperforms state-of-the-art pre-trained models (LayoutXLM, InfoXLMBase, and XLMRobertaBase) in 5, 6, and 7 out of 8 languages, respectively, improving the F1 score by 42% over LayoutXLM in English. To test the extensibility of the model, we further improve VRDSynth with automated table recognition, creating VRDSynth(Table), and compare it with extended versions of the pre-trained models, InfoXLM(Large) and XLMRoberta(Large). VRDSynth(Table) outperforms these baselines in 4 out of 8 languages and in average F1 score. VRDSynth also significantly reduces memory footprint (1M and 380MB vs. 1.48GB and 3GB for LayoutXLM) while maintaining similar time efficiency.

==> background.tex <==
%\subsection{Information Extraction from Visually Rich Documents}

%\subsection{Information Extraction from Visually Rich Documents}
%\label{subsec:bg_ie}
%\marc{what is key, value}
%\bachle{Give example. Also, define semantic and spatial relation. Don't expect readers to be familiar with those terms.}
%\subsection{Graph Neural Network}
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{images/e2eFlaxIE-GNN(1).jpg}
    \caption{Using Graph Neural Network to identify the desired fields, each text line, represented as a graph node in node-classification problem}
    \label{fig:gnn_ie}
\end{figure}

\textbf{Graph Neural Networks (GNNs)}. GNNs~\cite{Such2017, Zhang} are a class of neural network adapted for graph structures. In this work, we adapt the Chebyshev-approximation of Graph Convolution Network (GCN) as proposed in \cite{Zhang2016} and its variant to accommodate multiple types of edges as proposed in \cite{Such2017}. In order to employ GCN for documents IE, the document need to be transformed into a graph. The most common way for building graph from the document is to represent each segment as a node, the other information such as textual information, visual information are encoded as feature vector of the node. After the graph representation of document is generated, GCN is employed to incorporate graph's information, then the IE is formulated as graph node classification. 

\marc{How GNN is employed?}

%\subsection{GNN Explainer}
\textbf{GNN Explainer}. GNN explainer \cite{Cranmer2020} is a model-agnostic approach to provide explanation for GNN-based models. Explanation is provided under the form of adjacency and feature mask through an optimization process. GNN Explainer takes input as adjacency matrix, node features, a pre-trained model to optimize these masks.

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{images/MultiPerceptron-GNNExplainerOptimization.jpg}
    \caption{Modified GNN Explainer optimize masks on adjacency tensor: the size loss is used for minimizing size, the entropy loss ensure the mask's tendency to be closer to 0 or 1 while the consistency loss regulate the optimization to keep the prediction unchanged.}
    \label{fig:gnn_explainer_process}
\end{figure}

While the end-goal for explanation is to either debug or to interpret model output, we see that the given subgraphs and feature masks can be used to provide interpretable classification and used as materials to train program synthesis recognition model. 
For the problem of information extraction, we modified original GNN Explainer \cite{Crammer2020} to take input as an adjacency tensor and used 3 type of loss as in Figure \ref{fig:gnn_explainer_process}.

%\subsection{Explore/Compress/Compile}
\textbf{Domain Specific Language (DSL) and Program Synthesis.} The Explore-Compress-Compile ($\text{EC}^2$) is an algorithm to learns Domain Specific Language (DSL) and trains a recognition neural network for program searching\cite{Ellis}. $\text{EC}^2$ takes input as a set of tasks, and efficiently learns solving tasks progressively:
\begin{itemize}
 \item The Exploration phase consist of searching for program solving tasks under guiding of recognition model
 \item Compress refers to finding reused substructures among solved tasks and adding them to the library to reduce the search time for the next searches.
 \item Compile phase refers to training recognition model to guide the enumerative search.
\end{itemize}

\marc{make it concise}
Given a set of tasks, $EC^2$ framework is expected to gradually expand the library and solve the tasks in increased-complexity order.

In order to be able to expand the library, it is required that under the exploration steps a portion of tasks has to be solved.
The works currently focus on typical single-domain tasks such as text-editing, list-processing, etc. 
% We believe the ability to automatically leverages priors knowledge from solved program to learn DSL will be very useful in solving complicated problem of Information Extraction, given that the cost of designing tasks to capture domain-specific knowledge can be alleviated.

Our works aim to solve this gap by having the tasks automatically designed to capture GNN distilled knowledge to learn relevant reusable programs while boosting the performance of Information Extraction, this will be discussed in the next section.



==> draft_rl.tex <==

At initialization each variable's corresponding graph set are text line nodes in the document graph, the variable of which the graph started initialization with is called its root. 
We will start use the notation $GraphSet(v)$ to denote the set of graph that initialized with variable $v$.

Based on this observation, we first describe the algorithm in which the deletions of related nodes based on specified binary clause when a node does not match the next added clause.

Suppose that state $\mathscr{s}$  we have a graph set bound to variable $v$, which contain all the available nodes which are boundable this variable. 
We perform adding the clause to each graph, when the target nodes which available in this graph is not satisfied, they themselves are removed from this graph, the chain removals also occur if their related binary relation constraints has no other alternative bound nodes to match.
If their removal results in no bound nodes to any variable, the graph is deleted from the graph set.

When an unary clause is added, the satisfying condition is checked on each nodes which is bound to a variable in each graph.
When a binary clause is added, there might be two:
\begin{itemize}
    \item There exist a graph set in which both of the variables are added.
    \item There exist two graph set in which each variable is resided in one graph set.
\end{itemize}
In both of the case, the set of nodes for each variables are collected and first checked on the existence of corresponding nodes satisfying the relation, the unsatisfied ones are removed according to the specified removal procedure.
In the latter case, the clause is added to one graph set and two graph set are merged by the cached list of clauses.

% \marc{Theorem 0: The removing algorithm work exactly as desired.} 

% \marc{Theorem 1: At each state, there exist exactly one graph set that contains variable assignment}

% \marc{Theorem 2: All of the possible assignment are included}


The core of these procedure lies in 2 algorithms which leverage this architecture: 
The first is unary clause checking, the second is the graph merging algorithm to evaluate binary clause based on the conversion of an adjacency matrix to the list of node which is described in the next section.

==> experiment.tex <==
%\subsection{Information Extraction from Visually Rich Documents}
\section{Experiment}
\label{sec:experiment}
In this section, the effectiveness of \toolname is tested on several aspects, to answer the following questions:
\begin{itemize}
 \item The effectiveness of bridging algorithm ins booting the performance of program synthesis engine.
 \item The influence of synthesized rectifying program on the output of graph neural network 
 \item The performance of \toolname under unexplored and data deficient scenario.
\end{itemize}
These experiments will be demonstrated in the respective order below.
\subsection{Effectiveness of bridging algorithm}
In order to test the pre-training data effect on the reinforcement learning agent, a total of 10 fields in the Japanese invoice dataset is chosen.

\subsection{Synthesizing extraction program to rectify graph neural network's output}


\subsection{Performance under few-shot scenario}

\marc{Overall comments: The experiment sections better uses passive terms, or without subject, this is to enforce the notion of generalization/reproducability of them}
In this section we'll describe results from 3 experiments.
\subsection{Experiment Setup}

\subsection{Point 1: Effectiveness of pre-training compare to cold start (draft)}
We demonstrate the effectiveness of the bridging algorithm in closing the gap between the program synthesis engine and deep-learning based information extraction. In this experiment, we'll use half number of the fields for training, and the rest to verify the effectiveness of produced engine.

\subsection{Point 2: Performance improvement compare with previous methods (draft)}
\marc{The effectiveness of combining}
\subsection{Point 3: Transfer learning for few-shot information extraction (draft)}

==> important_related_works.tex <==
\cite{Sunder2019}
\textbf{dataset}
\cite{Jaume2019} Using Heuristic rules out perform model.
\marc{does deep learning + program synthesis out performs heuristic rules under FUNSD}?

\marc{And perhaps table decomposition?}


%\subsection{RL program synthesis}
\textbf{Reinforcement learning}. 

%\subsection{One-shot Information Extraction from Document Images using Neuro-Deductive Program Synthesis}
\textbf{One-shot Information Extraction from Document Images using Neuro-Deductive Program Synthesis}
\cite{Sunder2019} also target at extracting structured data from document images. This work use pre-trained deep learning models to populate entities and relations in document images. A resource-bounded meta-interpreter then is employed to construct proofs for the entities via logical deduction, and the proof is generalized to populate logical program.

%\subsection{Synthesis and Machine Learning for Heterogeneous Extraction}
\textbf{Synthesis and Machine Learning for Heterogeneous Extraction}
\cite{iyer2019synthesis} also propose an approach to combine machine learning and program synthesis to extract entities from heterogeneous data. Similar to \cite{Sunder2019}, a ML models is employed to get initial label of target fields. These noisy label are used as inputs to synthesis algorithm, generates a set of programs that be able to predict correct output. They then retain ML models and re-synthesize programs when there is disagreement between output of ML models and synthesized programs.


==> method_ProblemStatement.tex <==

\subsection{Graph-based information extraction} 
\label{subsec:graph_ie}

The base of our problem formulation is the representation of each document as a graph. Using this representation, we can either formulate the problem of information extraction as node classification on graph according to \cite{Liu2019} or using extraction program. Both of these formulations are important for our work which we will discuss below in respective order.

We use a representation of document $D$ as a graph $G$ similar to \cite{Liu2019}: By representing each text line as a node in graph and their spatial relations as graph edges. The construction of this representation is depicted as follows:

\textbf{Text line as graph node} We first construct a corpus of most frequently used characters and use them for bag-of-word encoding and normalize all the text line coordinates of each document to the range of $\left[0, 1\right]$ for uniformity. 
Under run time, each text line coordinates and content are produced by a text line recognition system (in our case, we employ a text-line segmentation\cite{Gruning2018} followed by Convolutional Recurrent Neural Network \cite{Shi2015}). Using this result, we produce final text line feature as concatenation of bag-of-words encoding and 4 spatial values $(x, y, w ,h)$ for their normalized coordinates, width and height respectively, we use bag-of-word encoding to encode each of text lines information, which we note to be a straight forward representation that can be explained directly via GNN Explainer \cite{Ying2019}.

\textbf{Relation construction} We use a projection-profile-based relation construction according to a few heuristics rule (see Figure ~\ref{fig:system_overview_inference} for example). Inspired from heuristic works which leverages relations by projection profile, the document graph leverage horizontal and vertical alignments between text lines of the document. If the projection profiles of two boxes overlap more than a certain threshold (we use 0.5), the two are considered as having a spatial relation to each other. In order for later step's interpretation of prediction, we prune the relations via another heuristic: no middle node with same relation allowed to exists between the two nodes under consideration.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{images/MultiPerceptron-HeuristicGraph.jpg}
%    \caption{The heuristic graphs built by considering the alignment between text lines, the red arrows represent left-right relation why the black arrows represent top-down relations}
%    \label{fig:heuristic_graph}
% \end{figure}

\textbf{Information extraction as node classification} Using graph representation, the information extraction from document image can be reformulated as node classification problem (see Figure \ref{fig:system_overview_training} and Figure \ref{fig:system_overview_inference}) where each node is classified to belong in one of $C$ categories. We employ this formulation along with labeled documents to train a GNN which is later used to boost the performance of program synthesis.

\textbf{Information extraction by program} We can also use the graph-based representation of document to facilitate information based on program, these programs take input as a graph $G$, choose a set of node as output for a specific category. As heuristic rules has been long used for information extraction from document image prior to deep-learning based method, we believe this line of direction has several potential on the interpretability and customizability, given that these rules can be generated in a data-driven manner. 
% One of the example program can be seen in Figure ~\ref{fig:gnn_rules_program_synthesis} and Figure ~\ref{fig:}, consisting of several logic constraints to extract the wanted entities. 

We also note that there exists alternative representation for this kind of program, including that of and other representation such as that of \cite{Huang2020} which allows grounding multiple entities at once directly, which we will demonstrate in Section ~\ref{sec:experiment}.




==> method_explainer.tex <==
\subsection{Explanation-based bridging between program synthesis and graph neural network}
\label{subsec:explanation}
In this subsection, we introduce the bridging algorithm to close the gap between program synthesis and graph neural networks.

This algorithm takes input as a set of labeled data (including set of targeting text lines) along with a trained Graph Neural Network model and produce example relational program for identifying multiple entities at once.

The algorithm transforming from explained adjacency mask of GNN explainer to program is straight forwards: based on breath-first search (BFS), we build an algorithm to convert from the mask to binary clauses and feature masks to unary clauses.

\begin{algorithm}
\SetAlgoLined
\KwResult{List clauses describing substructure}
\SetKwInOut{Input}{input}
\Input{
$A \in \{0; 1; 2; 3; 4\} ^ {N \times N}$: Quantized adjacency matrix obtained by combining masks of GNN Explainer. $A_{ij}$ describe having no relation, top, down, left, right \newline
$l\_box$ - List of document boxes with corresponding indices \newline
$l\_tgts$ - Indices of explained nodes. \newline
}
\Begin {
 $l\_clauses$ $\leftarrow$ $\left[\right]$\;
 $curr\_idxs \leftarrow l\_tgts$\; 
 $processed\_idxs$ \leftarrow $\left[\right]$\;
 \While{$len(curr\_idxs) > 0$}{
    i = $curr\_idxs.pop(0)$\;
    $next\_idxs \leftarrow NonZeroIndices(A[j, :])$\;
    \For{$j \in next\_idxs$}{
        $l\_clauses.append(
            BinaryClause(binary_rel[A[i, j] - 1], i, j)
        )$\;
        $A[i, j] = 0$\;
        $A[j, i] = 0$\;
    }
    $processed\_idxs.append(i)$\;
    $curr\_idxs \leftarrow Union(curr\_idxs, next\_idxs) $
 }
 $l\_clauses \leftarrow$ Rename($l\_clauses$, $processed\_idxs$)\;
 \Return $l\_clauses$\;
 }
 \caption{Getting binary clauses from highlighted adjacency matrix}
 \label{algo:bin_clauses}
\end{algorithm}

\begin{algorithm}
\SetAlgoLined
\KwResult{List unary clauses for each variable}
\SetKwInOut{Input}{input}
\Input{
$processed\_idxs$: List of corresponding boxs' indices in the original document graph
$F \in \{0; 1\}^ {N \times F}$: List of highlighted features for each box
}
\Begin{
  $l\_uclauses \leftarrow \left[\right]$\;
  \For {$orig\_idx, p\_idx) \in enumerate(processed\_idxs)$}{
    \For {$idx \in NonZeroIndices(F[orig\_idx, :])$}{
        $l\_uclauses.append(p\_idx, feature(idx))$\;
    }
  }
  \Return $l\_uclause$\;
}
\caption{Getting unary clauses from highlighted features}
\label{algo:unary_clauses}
\end{algorithm}

$F \in \{0; 1\} ^ {N(N_w + 4)}$ obtained by thresholding GNN Explainer masked feature, describe whether a feature is important to the prediction. \newline
$C$ - Corpus - list of chosen words from data.


Using this algorithm, we can also try specifying multiple target fields, these referring programs can also be used directly as template for matching or information extraction between forms.

These structures contain necessary information as well as common type of relations which are most important for Graph Neural Network, thus, helping us distill the trained network's knowledge to train the Reinforcement Learning model.

To use this, we ran each program produced by this process via action execution engine mentioned earlier to produce feedback to agent. 
Note the program does not guaranteed to be accurate, but the experience can still be distilled to the agent.

==> method_overview.tex <==
We bridge the performance gap between Graph Neural Network (GNN) and Program synthesis by converting the output of pre-trained GNN model to a set of relational program and automatically generate extraction programs, which are expected to take input as a document graph and extract desired entities.

Using these relational rules, we generate tasks for a reinforcement-learning based program synthesis engine to learn from.
By adopting GNN distilled extraction program, the engine is expected to be able to produce more complex program.
The learned program synthesis engine is then used either to adapt to newly annotated fields in an interpretable and optionally can be guided by user.

These training stages is depicted in Figure \ref{fig:system_overview_training}, where we divide the training into 3 stages: data generation, pre-training (bridging) and reinforcement learning training.

At inference time, the architecture of the resulting system is depicted in Figure \ref{fig:system_overview_inference}, where the learned Graph Neural Network is combined with the discovered supplemental programs to output the final results.

% Our system \toolname combines deep learning and program synthesis to effectively generate programs that can accurately extract relevant information from documents.
% Document images are first decomposed into a set of text lines and their coordinates. 
% Afterwards, \toolname transforms the text lines and coordinates into graph-based representation. 

In Subsection \ref{subsec:graph_ie} we describe the problem formulation of information extraction based on graph representation, along with explanation of how program synthesis can be applied as a mean for find desired entities. We continue describe the synthesis engine in Subsection ~\ref{subsec:method_rl}. 
Finally, we depicts how to bridge the performance between a trained graph neural network and the program synthesis engine in Subsection ~\ref{subsec:explanation}.

==> method_rl.tex <==
\subsection{Reinforcement-learning based program synthesis for information extraction}
\label{subsec:method_rl}

In this subsection, we describe our usage of a reinforcement learning model to solve the problem of finding extraction programs. 
We follow \cite{Huang2020} and formulate the problem of information extraction as a referring relation program, this is due to several observations:
\begin{itemize}
    \item We see the analogy between using referring expression to ground object based on a graph of constructed relation and the use of extraction program to find desired entities.
    \item Hypothetically, the generation of each part of program as referring clause to be evaluated as an intermediate feedback of reinforcement learning may allows pruning of unnecessary branch, thus, speed up the search.
\end{itemize}
In order to leverage the reinforcement learning, we will discuss the detailed problem formulation, along with other required aspect such as the model, the rewards function and the inference engine of these program.

\textbf{Formal Definitions}

Given a set of document graph - target pairs $\{G, T\}$, where each document graph $G$ is defined as a tuple of $(V, A)$ of nodes and adjacency tensor as defined above and target set $T \subset V$ is a set of nodes that need to be grounded, the goal of the agent is finding a program which can match the document graphs to corresponding targets.


The programs are written in logic language according to \cite{Chen2019a} (depicted in Figure \ref{fig:referring_entity_program}), each program is consist of a set of variables $Var$ and constraints $C$, where each $var$ is a variable that can be assigned to any text line satisfying group constraints, the determination of variables to text lines mapping will be later in this section.
In detail, a constraint is specified via a clause, either unary clause or binary clause, we list the types of clauses shortly:
\begin{itemize}
    \item Unary clauses consist of constraint on the property of an individual variable and its corresponding assigned node, of which we have two types of unary clause, containing of character or spatial property. For example: $c\langle i \rangle(var0,\ 'True')$ specify the containing of $i$th character in the corpus of the nodes assigned to $0$th variable, while $down\_most(var0,\ 'True')$ specify the constraint that nodes assigned to $var0$ must not contain any nodes below it according to the heuristic graph.
    \item Binary clauses consist of constraint on relation between two variables' assigned nodes: $down(var0,\ var1)$ means that nodes assigned to $0$th variable must exists some neighbors in downward direction according to the heuristic rules which are assigned to $1$th variable.
\end{itemize}

Next, we discuss the components of the reinforcement learning framework as stated in Figure \ref{fig:rl_overview}. 
In our case, the synthesizer itself it a reinforcement learning agent, of which we applied the same Q-learning framework which used in the work of \cite{Huang2020}, according to Figure \ref{fig:rl_overview}, 3 components are needed for the framework: the value network, action execution engine and the reward. We will discuss each of these components below.
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\textwidth]{images/RLTraining.png}
%     \caption{The reinforcement learning consists of 3 main components: the policy networks, the inference engine, and the rewards}
%     \label{fig:rl_overview}
% \end{figure}
\textbf{Value Network}
Given the input as encoded information of state and necessary environment properties, the value network output the predicted score of each actions.
From these output, an action will be chosen by the agent to interact with the environment. The detailed model description can be seen in Figure \ref{fig:rl_model}.
The value network is trained using feedback from the environment according to standard Deep Q-Learning training.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\textwidth]{images/MultiPerceptron-RLModel2(2).png}
    \caption{First, the state information is splitted into 2 input streams: program state and graph state which are forwarded through 2 slightly different set of GNN layers because the program state requires less complexity functions to proceed than the graph information. Then, the concatenation of the outputs is used as the initial hidden state alongside with the action embedding as the input sequence of a recurrent neural network (RNN). The final output extracted after several linear layers is the predicted value of the state-action pair. 
}
    \label{fig:rl_model}
\end{figure}

\textbf{Action Execution Engine} As one integral part of the environment, the action execution engine takes output of the value network and interact with the environment so that the next state can be received for the agent to improve.
In our case, the execution engine would take input clauses such as $c150(var0,\ 'True')$ or $down(var0,\ var1)$ and calculate possible assignments for each variables, in other words, it has to filter unsatisfied candidates given the constraints.
For this task, it might be straight forward to implement an exhaustive search similar to the inspired work of \cite{Huang2020}, we have found limitations when applying the same strategy in our scenario:
In \cite{Huang2020}, the method implemented listing all possible mapping from each variable to each entities, in our scenario, it is the same as defining the mapping $s_0: Var \mapto V$ at initialization, for example: if we have $var0$ and $var1$ along with 7 entities, there would be $7^2$ possible combinations: $(0, 0), (0, 1), \cdots, (6, 6)$, each is a possible assignment from variable to an object.
After each constraint is added (see Figure \ref{fig:referring_entity_program}), the previous execution engine loops through all the remaining combinations and filters out the unsatisfying ones. 
At the scale of previous settings, the size of $O(|V|^{|Var|)}$ does not seems to pose much problem, however, under our scenario, where the maximum number of text lines might reach over 100 and the required variable from GNN explainer can be up to 12, the brute force approach poses serious problem in computational and memory complexity.

Thus, we have decided to implement a different approach to realize the action execution engine. First, we made the following observations:
\begin{itemize}
    \item The exhaustive state space includes all the possible combinations of entities for variable assignment.
    \item In reality, few entities are suitable at each time step to be assigned.
    \item When an unary clause is added, only filtering occurs (The number of assignment in the state matrix is decreased).
    \item When a binary clause is added, it might be the new variable is added and new edge that connects between variables are added, making the memory consumption increase.
\end{itemize}
Thus, we have decided to keep the memory bounded by decoupling variable assignment at the beginning while gradually merge group assignment as binary clauses are added and candidates are filtered:
\begin{itemize}
    \item At the begining, each variable is assigned to all possible entities, we keep track of mapping between variable to entities in form of a dictionary.
    \item As binary clauses are added, these group of variable assignments are merged together while unsuitable candidates are filtered.
    \item At any time, if a node fails to satisfy an added constraints, a group instance is removed.
\end{itemize}

A node is satisfied with an unary clause when its own property is matched with the clause, and is satisfied with a binary clause if and only if there exists other nodes which can satisfies the other conditions and have the corresponding relations with this node.
We keep track of the possible assigment of variable-node assignmennt at all time step to provide rewards for the agent as decribed below.

\textbf{Rewards}
At any given timestep $t$, the reinforcement learning agent receives the variable-objects mapping state $s_t: Var \mapto V$ indicating the set of objects which a variable can be assigned to.

Given this settings, the total rewards that the agent receives is as follows:
\begin{equation}
    R = R_{precision} + R_{completion} - P_{recall} - P_{length} 
\end{equation}
Where:
\begin{itemize}
    \item $R_{precision}_t = \sum_{var} |s_t(var) \setminus s_{t-1}(var) \setminus T| / |V|$ is calculated reduction ratio on non-relevant objects. For example, let $var0$ target the field $company\_name$, then the precision rewards will be calculated as total reduction of other fields' object assigned to $var0$.

    \item $R_{completion} = r_c |V| / |T|$ where $r_c$ is a hyper-parameter, the completion reward is triggered after the success grounding of target objects at the end of each episode.
    \item $P_{recall}$ is fixed to $1$ and is triggered when an episode is ended by ruling out any target variable.
    \item $P_{length}$ is a fixed constant ($0.1$ in our case) to prevent the length of each program.
\end{itemize}

In short, we give rewards when irrelevant nodes are removed or the grounding is completed and penalize if the wanted node is removed or program length increases.

Similar to \cite{Huang2020} we also employ enumeration-based program synthesis like \cite{Nye2019a} when the length of program reaches a certain threshold.

\hector{move to Exp setup}
\textbf{Synthesizing program for extraction from scratch} To synthesize the program from scratch, we take input as an unlabeled document graph then try finding programs which correct covers a maximum set of text lines which belong to each fields.

\textbf{Synthesizing program for extraction based on previous prediction} In order for program synthesis to complement GNN output, we train program to ground two fields at the same time so that at run time, we may propagate from highly-confidence fields of GNN output to uncertain fields using these program.In \cite{Huang2020}, the method implemented listing all possible mapping from each variable to each entities, in our scenario, it is the same as defining the mapping $s_0: Var \mapto V$ at initialization, for example: if we have $var0$ and $var1$ along with 7 entities, there would be $7^2$ possible combinations: $(0, 0), (0, 1), \cdots, (6, 6)$, each is a possible assignment from variable to an ob



==> related_works.tex <==
%\kai{It is better to discuss previous work. What are drawbacks and conclude by why this research is important}

%\marc{In order to incorporate both spatial and semantic information, recent works have also modeled the problems as semantic segmentation over different representations \cite{Katti2018, Madashi2019} and link-classification over nodes for table structure extraction \cite{Qasim}. }
This section describes recent state-of-the-art approaches in information extraction (IE) based on template matching~\cite{field_extraction_document_images_Rusinol2013}, feature engineering heuristics~\cite{Ahn2017,Bukhari2011}, deep learning~\cite{Liu2019}, and program synthesis~\cite{Sunder2019,Iyer}.

%\subsection{Traditional Information Extraction}
Template matching based IE approaches require substantial effort to categorize documents into templates~\cite{field_extraction_document_images_Rusinol2013}. Documents can be clustered based on visual and textual similarity. For visual similarity, perceptual hashing can be used to calculate the similarity between a given template and a target document image, e.g., \cite{chum2008near}. For textual similarity, Levenshtein edit distance is the best known choice \cite{yujian2007normalized}. These approaches are, however, arguably not scalable and tractable due to the rising complexity of templates when new documents come along. In reality, there could be thousands of business vendors having varying forms of documents, making the management of templates easily become intractable, e.g., checking for duplication of templates is error prone. Furthermore, template-based approaches are also prone to varying visual quality of documents. For example, document images with low visual quality may unduly be classified as new templates, rendering template-based approaches imprecise.

Heuristic-based IE methods rely on carefully designed feature engineering to reconstruct visually rich documents as components~\cite{Ahn2017, Bukhari2011}, allowing for queries on individual component to extract desired information. 
Examples of the designed features include the use of ridges and white-spaces~\cite{Bukhari2011} or connected component analysis~\cite{Ahn2017} to decompose images into text line segments. Heuristic rules can then be derived to query the segments for desired fields, e.g., text fields are tagged~\cite{ciravegna2001adaptive} for ease of queries. Unfortunately, similar to template-based approaches, heuristic-based approaches suffer from intractability and scalability. The manually crafted features and rules may highly overfit specific forms of documents, rendering heuristic-based approaches to be less generalizable across a diverse set of documents in practice.


%\subsection{Graph Convolution Network}
Deep learning has recently been used for IE to overcome the limitations of template matching and heuristic-based approaches.

% \bachle{Please look at Section 2.1 and 2.2 in the~\cite{Liu2019} paper to identify more related work such as deep learning based approaches for IE. I will edit after you write it here}.

For information extraction from visually rich documents (VRD), the closest work to ours is \cite{Palm2018} where they use a recurrent neural network (RNN) to extract entities using textual features. Unfortunately, with the limitation of RNN, they have ignored the contribution of image features and heavily relied on the left-to-right reading order. Additionally, \cite{d2018field} adds more hand-crafted features such as the the invoice number is on the same line, on the left of the word 'facture' to model the semantic spatial relationship between entities which is not scalable in the real-world applications. Besides, \cite{Katti2018} provides a generic document understanding using CNN to predict a segmentation mask called 2D chargrid that indentify the text characters and the bounding boxes. Nevertheless, 2D chargrid or segmentation based IE methods usually don't work in the case of dense documents with little spaces between entities. Although both CNN and RNN can vastly bridge the gap between computer program and human capability to extract information from documents, they has proven insufficient to deal with complex structure documents.

Recently, Graph Convolution Network (GCN) \cite{kipf2016semi} \cite{hamilton2017inductive} has started a surge of interest in extracting information from complex structure like social networks, chemical formulae .Additionally, by formulating an input as a document graph, \cite{Peng2017} \cite{song2018n} introduces graph LSTM and graph-state LSTM to extract the cross-sentence relations of n sentences. On the other hand, to model the visual context, \cite{Liu2019} introduced  edge embedding into the graph convolution network to model the relationship between vertices. \cite{Qasim} introduce a standard pipeline for IE using GCN with visual feature extraction using CNN and vertex interaction with different choices of GCN such as \cite{Qasim2019} and \cite{Wang2019}. Even though GCN has overcome the weakness of previous methods, unlike heuristic methods, it has a strong prone to overfit the superficial graph structures ignoring the true meaning of the relationship between vertices.


%GCN is chosen due due to its ease of implementation and lightweight \cite{Such2017}, making it a decent candidate under data-deficient condition which is often the case in complicated data such as visually-rich-documents (requiring annotations of all text lines coordinates and their content)
As a result, to fill in the holes left by GCN, entity referring expressions are necessary. By previously proving that expressions from heuristic methods are insufficient and less generalizable, we introduce a perfect alternative called program synthesis. \cite{Nye2019a} learning an intermediate ‘sketch’ representation to later perform symbolic search to find a program satisfying the spec. Recent work~\cite{Iyer} uses conditional random field and disjunctive program synthesis together for heterogeneous extraction. However, their approach is specifically designed for expert users who can manually write a domain specific language (DSL) as input to program synthesis, rendering the approach less reusable and unfriendly to non-expert end users. 
 
In this work, instead of totally relying on GCN and requiring user to write DSL, we use the rule set from program synthesis to detect information from document patches that are usually failed with GCN. Different from existing works, in this paper, we use program synthesis to automatically generate rules including graph traversal and those belong to heuristic methods. Thus, this approach vastly reduces chance of overfitting from the manually design rules and increase the scalability at the same time.



==> rl_background.tex <==
First, to adapt reinforcement learning to our problem, we begin by formalize our problem as a Markov Decision Process (MDP) $\matchscr{M} = (\matchscr{S}, s_0, \matchscr{A}, \matchscr{R}, \matchscr{T}, \gamma)$ where:
$\matchscr(S)$ is a set of states, 
$s_0$ is a fixed initial state,
$\matchscr{A}$ is a set of discrete actions,
$\matchscr{R}: \matchscr{S} \times \matchscr{A} \rightarrow \mathbb{R} $ is the reward function,
$\matchscr{T}: \matchscr{S} \times \matchscr{A} \times \matchscr{S} \rightarrow [0, 1]$ is the transition dynamics of the environment and
$\gamma \in [0, 1]$ is the discount factor 


==> suplementary_material.tex <==
%\subsection{Information Extraction from Visually Rich Documents}
%\label{subsec:bg_ie}
%\marc{what is key, value}
%\bachle{Give example. Also, define semantic and spatial relation. Don't expect readers to be familiar with those terms.}
In this section, we formally define the information extraction (IE) problem from virtually rich documents (VRDs) following~\cite{Madashi2019, Jaume2019} and subsequently provide the background on constituent parts of \toolname that we use. In particular, we will describe Graph Neural Networks (GNNs)~\cite{} that learn to represent VRDs as graphs, GNN Explainer~\cite{} that explains the models learned from GNNs, and a DSL and program synthesizer~\cite{} used to synthesize programs that rectify errors of the GNN's model.

\begin{definition}
Information Extraction. Visually rich documents (VRDs) can be represented as text segments, each of which contains text content and the bounding box of the segment. Let a VRD be defined as a set of $N$ text segments $\langle t_i \rangle$. Each segment $t_i$ is represented as a tuple of $(x, y, w, h, text)$ which denotes coordinates of the segment in the VRD, the width, height and content of the segment respectively. Given $f$ denoting the desired field to extract from a VRD, information extraction outputs a set of text segments $\langle t_f \rangle$ which are associated with the desired field $f$.
\end{definition}

In this work, we represent each VRD as a graph, wherein each node represents a text segment and an edge between two nodes represents the spatial relation among the nodes, e.g., the relative position (alignment) between the nodes' text segments on the VRD. Nodes that share some common property can be categorized into groups. The IE problem is now equivalent to the problem of querying graphs to retrieve relevant group of nodes associated with a desired property $f$. To achieve this, we use a Graph Neural Network (GNN) to learn a model for node classification. We next explain the GNN that we use~\cite{Such2017} which enables to incorporate both semantic and spatial relations among nodes.

\textbf{Graph Neural Networks (GNNs)}. GNNs~\cite{Such2017, Zhang} are a class of neural network adapted for graph structures. In this work, we adapt the Chebyshev-approximation of Graph Convolution Network (GCN) as proposed in \cite{Zhang2016} and its variant to accommodate multiple types of edges as proposed in \cite{Such2017}. In order to employ GCN for documents IE, the document need to be transformed into a graph. The most common way for building graph from the document is to represent each segment as a node, the other information such as textual information, visual information are encoded as feature vector of the node. After the graph representation of document is generated, GCN is employed to incorporate graph's information, then the IE is formulated as graph node classification. 

\marc{How GNN is employed?}

%\subsection{GNN Explainer}
\textbf{GNN Explainer}. GNN explainer \cite{Cranmer2020} is a model-agnostic approach to provide explanation for GNN-based models. Explanation is provided under the form of adjacency and feature mask through an optimization process. GNN Explainer takes input as adjacency matrix, node features, a pre-trained model to optimize these masks.

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{images/MultiPerceptron-GNNExplainerOptimization.jpg}
    \caption{Modified GNN Explainer optimize masks on adjacency tensor: the size loss is used for minimizing size, the entropy loss ensure the mask's tendency to be closer to 0 or 1 while the consistency loss regulate the optimization to keep the prediction unchanged.}
    \label{fig:gnn_explainer_process}
\end{figure}

While the end-goal for explanation is to either debug or to interpret model output, we see that the given subgraphs and feature masks can be used to provide interpretable classification and used as materials to train program synthesis recognition model. 
For the problem of information extraction, we modified original GNN Explainer \cite{Crammer2020} to take input as an adjacency tensor and used 3 type of loss as in Figure \ref{fig:gnn_explainer_process}.

%\subsection{Explore/Compress/Compile}
\textbf{Domain Specific Language (DSL) and Program Synthesis.} The Explore-Compress-Compile ($\text{EC}^2$) is an algorithm to learns Domain Specific Language (DSL) and trains a recognition neural network for program searching\cite{Ellis}. $\text{EC}^2$ takes input as a set of tasks, and efficiently learns solving tasks progressively:
\begin{itemize}
 \item The Exploration phase consist of searching for program solving tasks under guiding of recognition model
 \item Compress refers to finding reused substructures among solved tasks and adding them to the library to reduce the search time for the next searches.
 \item Compile phase refers to training recognition model to guide the enumerative search.
\end{itemize}

\marc{make it concise}
Given a set of tasks, $EC^2$ framework is expected to gradually expand the library and solve the tasks in increased-complexity order.

In order to be able to expand the library, it is required that under the exploration steps a portion of tasks has to be solved.
The works currently focus on typical single-domain tasks such as text-editing, list-processing, etc. 
% We believe the ability to automatically leverages priors knowledge from solved program to learn DSL will be very useful in solving complicated problem of Information Extraction, given that the cost of designing tasks to capture domain-specific knowledge can be alleviated.

Our works aim to solve this gap by having the tasks automatically designed to capture GNN distilled knowledge to learn relevant reusable programs while boosting the performance of Information Extraction, this will be discussed in the next section.


\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{images/MultiPerceptron-GNNArchitecture(2).jpg}
    \caption{Employed Graph Neural Network Architecture, $GConv$ is the graph convolution layer, $Embedding$ is a linear layer per node feature, $Concat$ concatenate node-wise features}
    \label{fig:gnn_architecture}
\end{figure}

\textbf{Architecture: } After all text line features are extracted and the document graph is built, we employed a GNN Architecture of total 5 Graph Convolution (GCN) Layer \cite{Kipf2017, Such2017} in Figure \ref{fig:gnn_architecture}, each are activated by ReLU activation \cite{AlexNet}. Skip connections are also used under the form of concatenation to facilitate gradient flows during training. 
The final layer is an embedding layer to map from per-node aggregated features to available classes.


==> supplement_rtree.tex <==
\textbf{Graph-based Information Extraction Explanation Via Rules: } We convert GNN Explainer output (adjacency mask and feature masks of nodes) into recognition rules of text lines via the algorithm described in Algorithm \ref{algo:tree_path}. The resulting tree contains keywords as well as children set based on spatial relations is used to be converted to rule in Algorithm \ref{algo:tree_path_to_rule}.


\kai{what are keyword and children? is it key-values?}

\kai{explain algorithm 1 and 2 by words, about how they performs the task. Pseudo code is not the best way to explain idea. For example, how to obtain rules from gnn explainer results. 
Also, algo2 sub-function can be named for easy understanding like text(x), boundingbox(x) then can skip definition mappings. What is the role of lefts, rights, tops, downs?} 


\begin{algorithm}
\SetAlgoLined
\KwResult{Relation Tree from main node}
\SetKwInOut{Input}{input}
\Input{
$A \in \{0; 1; 2; 3; 4\} ^ {N \times N}$: Quantized adjacency matrix obtained by combining masks of GNN Explainer. $A_{ij}$ describe having no relation, top, down, left, right \newline
$F \in \{0; 1\} ^ {N(N_w + 4)}$ obtained by thresholding GNN Explainer masked feature, describe whether a feature is important to the prediction. \newline
$C$ - Corpus - list of chosen words from data.
$l\_box$ - List of document boxes with corresponding indices \newline
$i$ - Index of explained node. \newline
}
\Begin {
 $l\_rtree$ $\leftarrow$ $\left[new\ \mathbf{RTree}\ \textbf{for}\ box \in l\_box\right]$\;
 $l\_widx$ $\leftarrow$ GetWordIndices($F[i] == 1$)\;
 $l\_rtree[i].kwrds$ $\leftarrow$ [$C[w\_idx]$ \textbf{for} $w\_idx$ $\in$ $l\_widx$]\;
 $mask\_taken \leftarrow$ $\left[False\ \textbf{for}\ box \in lbox\right]$\;
 $curr\_idxs \leftarrow [i]$\; $mask\_taken[i] \leftarrow True$\;
 \While{$len(curr\_idxs) > 0$}{
  $next\_idxs \leftarrow []$\;
  \For{$j \in curr\_idxs$}{
    \For{$k \in NonZeroIndices(A[j, :])$}{
        \If{\Not{$mask\_taken[k]$}}{
            $next\_idxs.append(k)$\;
            $l\_rtree[j].children[A[j, k] - 1].append(l\_tree[k])$\;
            $mask\_taken[k] \leftarrow True$\;
        }
    }
  }
  $curr\_idxs \leftarrow next\_idxs$\;
 }
 \Return $l\_rtree[i]$\;
 }
 \caption{get\_rtree: Getting Tree Paths from main node}
 \label{algo:tree_path}
\end{algorithm}

After the tree paths is obtained, we proceed converting sample to rule in Algorithm \ref{algo:tree_path_to_rule}.

\begin{algorithm}
\SetAlgoLined
\KwResult{Lambda function to match with a text line}
\SetKwInOut{Input}{input}
\Input{$rtree$ - Relation Tree from the main node}
\Begin{
 $l\_action \leftarrow [0; 1; 2; 3]$
 $l\_act\_func \leftarrow [traverse\_left, traverse\_right, traverse\_top, traverse\_down]$\;
 $rule \leftarrow \lambda\ x:True$\;
 \For{$kw in rtree.kwrds$}{
    $new\_sub\_rule \leftarrow \lambda\ x: contain\_text(get\_text(x))(kw)$\;
    $rule \leftarrow \lambda\ x: and(rule(x)) (new\_sub\_rule(x))$\;
 }
 $rel\_rule \leftarrow \lambda\ x: True$\;
 \For{$action \in l\_action$}
 {
    \For {$child \in rtree.children[action]$}{
        $rel\_rule\ \leftarrow \newline 
        \lambda\ x:and(rel\_rule(x))( \newline
        \quad any(get\_rule(child))(l\_act\_func(x)) \newline
        )$\;
    }
 }
 \Return $rule \leftarrow \lambda\ x: and(rule(x))(rel\_rule(x))$\;
}
\caption{get\_rule: Converting from tree path to rule}
\label{algo:tree_path_to_rule}
\end{algorithm}


In order to overcome this, we employ post-processing rules synthesized from a deep-learning augmented program synthesis, since the rule-synthesizer is trained across different tasks, it is expected to be able to distill learned rules across tasks, giving a boost in performance.
\marc{Better have a grammar}
\marc{At the begining of each task: What is the goal of each task, then, to achieve this goal, we design these tasks}.
\marc{The goal of this rule-learning and synthesis is to achieve...}
\marc{Use examples instead}
\marc{Each time when we refer to smt in Background, mention it in introduction and explain its purpose}
We formulate the problem of information extraction task for program synthesis as follows:
Given a set of $N$ text lines $\langle t_i \rangle_{(N)}$  represented as tuple of $(id, x, y, w, h, text, tops, downs, lefts, rights)$ for the index in list, coordinates, its text content and lists of related ids respectively, we denote this type of tuple $TDocumentBox$. $id$ is of type $TInt$, while $x, y, w, h$ are of type $TReal$, $text$ is of type $TList(TChar)$ (text is a list of characters) and 
Output is a list of boolean $\langle o_i \rangle_{(N)}, o_i \in \{True, False\}$ for each of the desired fields indicating whether each text line belong to the desired class.
In order to do this, we facilitate the set of primitive lambda function as follows:
\begin{itemize}
    \item $traverse\_left$, $traverse\_right$, $traverse\_top$, $traverse\_down$: $(TDocumentBox, TList(TDocumentBox)) \rightarrow TDocumentBox$: This take a document box and a list containing all text lines belong to a document and get the nearest related box, if there does not exist any related box in the direction, the function return $NULL$.
    \item $get\_text: TDocumentBox \rightarrow TList(TChar)$ get the text content of a text line, will return an empty list if the text line is $NULL$.
    \item $get\_x, get\_y, get\_w, get\_h: TDocumentBox \rightarrow TReal$ get the property of the text line, if given $NULL$ these function will return $-1.0$.
    \item $contain\_char: (list(TChar), Tchar)  \rightarrow TBoolean$ checking whether a text content contains a character.
    \item $greater, equal: (TReal, TReal) \rightarrow TBool$ checking whether a real value is greater than or equal another.
    \item $and, or: (TBoolean, TBoolean) \rightarrow TBoolean; not: TBoolean \rightarrow TBoolean$ - logical functions to combine conditions.
    \item $map: (TVar0 \rightarrow TVar1, TList(TVar0)) \rightarrow TList(TVar1)$ mapping from one type of list to another.
\end{itemize}

